Seven decades of exploring planetary interiors with rotating convection experiments

The interiors of many planets consist mostly of fluid layers. When these layers are subject to superadiabatic temperature or compositional gradients, turbulent convection transports heat and momentum. In addition, planets are fast rotators. Thus, the key process that underpins planetary evolution, the dynamo action, flow patterns and more, is rotating convection. Because planetary interiors are inaccessible to direct observation, experiments offer physically consistent models that are crucial to guide our understanding. If we can fully understand the laboratory model, we may eventually fully understand the original. Experimentally reproducing rotating thermal convection relevant to planetary interiors comes with specific challenges, e.g. modelling the central gravity field of a planet that is parallel to the temperature gradient. Three classes of experiments tackle this challenge. One approach consists of using an alternative central force field, such as the electric force. These are, however, weaker than gravity and require going to space. Another method entails rotating the device fast enough so that the centrifugal force supersedes Earth's gravity. This mimics the equatorial regions of a planet. Lastly, by using the actual lab gravity aligned with the rotation axis, insight into the polar regions is gained. These experiments have been continuously refined during the past seven decades. We review their evolution, from the early days of visualising the onset patterns of convection, over central force field experiments in spacecrafts, liquid metal experiments, to the latest optical velocity mapping of rotating magnetoconvection in sulfuric acid inside high-field magnets. We show how innovative experimental design and emerging experimental techniques advanced our understanding and painted a more realistic picture of planetary interiors, including Earth's liquid metal outer core.

==> CR-gen.tex <==
% We want to compile old articles (issues up to 2023) using the old template.
% Since the publication date is set in the .cfg file loaded after CR-gen.tex, we
% need to postpone the detection. It makes some of the code a bit heavier, but
% it is better than breaking everything.

\newif\ifcdr@oldtemplate
\ExplSyntaxOn
  \AtBeginDocument{
    \int_compare:nT {1 < \currentyear < 2024} {\cdr@oldtemplatetrue}
    \ifcdr@traduction \cdr@oldtemplatefalse \fi
    \ifcdr@oldtemplate
      \definecolor{cdr@accentcolor}{rgb}{0,0.6,.4} % AcademyGreen
    \fi
  }
\ExplSyntaxOff

\ifcdr@epreuves\RequirePackage[angle=60,scale=1.5,text={}]{draftwatermark}\fi
\ifcdr@epreuves\RequirePackage[pagewise,mathlines]{lineno}\fi
\ifcdr@traduction\RequirePackage[fitting,skins]{tcolorbox}\fi
\RequirePackage[absolute]{textpos}
\RequirePackage{cedram-graphics}
\RequirePackage[french,english,iso,cleanlook]{isodate} \origdate
\RequirePackage[shortlabels]{enumitem}

\def\currentjournaltitle{Comptes Rendus. \CDRcrasseries}
\def\currentjournalpublisher{Acad\'emie des sciences, Paris}
\def\journalURL{https://comptes-rendus.academie-sciences.fr/\cdr@journaldirectory/}%

\definecolor{cdr@accentcolor}{RGB}{125,103,255} % AcademyPurple

\let\cdr@rubricFR\@empty
\let\cdr@rubricEN\@empty
\let\cdr@presentedby\@empty
\let\cdr@resps\@empty
\let\cdr@specialtitle@english\@empty
\let\cdr@specialtitle@french\@empty

\def\cdr@printer@fr{}%{Imprim\'e en France par Sud Light Production / Clip (Centre Litt\'eraire d'impression Proven\c{c}al), Marseille, France}
\def\cdr@printer@en{}%{Printed in France by Sud Light Production / Clip (Centre Litt\'eraire d'impression Proven\c{c}al), Marseille, France}

\def\TopicFR#1{\gdef\cdr@topicFR{#1}}
\def\TopicEN#1{\gdef\cdr@topicEN{#1}}
\def\TopicEF#1#2{\gdef\cdr@topicEN{#1}\gdef\cdr@topicFR{#2}}
\def\RubricEF#1#2{
  \ClassError{cedram}{\noexpand\RubricEF is deprecated, use \string\CDRsetmeta{articletype}}{}
}

\ifcdr@LTXGrid
  \RequirePackage[papersize={192mm,262mm}, hmargin=16mm, vmargin={26.9mm,24.7mm}, foot=14mm, head=10pt, headsep=10mm]{geometry}
  \skip\footins=18ptplus12pt
  \abstractmargin6em
  \parskip0ptplus.1pt
  \floatsep 12pt plus 2pt minus 2pt
  \textfloatsep 20pt plus 2pt minus 4pt
  \intextsep 12pt plus 2pt minus 2pt
  \dblfloatsep 12pt plus 2pt minus 2pt
  \dbltextfloatsep 20pt plus 2pt minus 4pt
  \@fptop 0pt plus 1fil
  \@fpsep 8pt plus 2fil
  \@fpbot 0pt plus 1fil
  \@dblfptop 0pt plus 1fil
  \@dblfpsep 8pt plus 2fil
  \@dblfpbot 0pt plus 1fil
  \partopsep 2pt plus 1pt minus 1pt
  \def\clearlastpage@hook{\onecolumngrid\clearpage\eject}
  \def\@makefntext{\rule{0pt}{14pt}\@makefnmark}
\else
  \RequirePackage[papersize={192mm,262mm}, vmargin={26.9mm,24.7mm}, hmargin=26mm, foot=14mm, head=10pt, headsep=10mm]{geometry}
  \abstractmargin2em
\fi

\skip\@mpfootins=\skip\footins
\columnsep=18pt
\columnseprule=0pt
\abstractmarginL\abstractmargin
\abstractmarginR\abstractmargin
\marginparsep=10pt
\marginparpush=5pt
\marginparwidth=20mm
\pretolerance=600
\tolerance=2400 % INITEX sets this to 10000
\hbadness=2500
\vbadness=1000
\linepenalty=10
\hyphenpenalty=40
\exhyphenpenalty=50
\binoppenalty=700
\relpenalty=500
\clubpenalty=3000
\widowpenalty=4000
\displaywidowpenalty=6000
\brokenpenalty=3000
\predisplaypenalty=10000
\doublehyphendemerits=600
\finalhyphendemerits=4000
\adjdemerits=10000
\emergencystretch=1.5em
\uchyph=1
\hfuzz.5pt
\lineskip=0pt
\normalparindent=12pt
\parindent=\normalparindent
\captionindent=\normalparindent

\def\@mainsize{10}
\def\@ptsize{0}
\def\@typesizes{%
  \or{5}{6}\or{6}{7}\or{7}{8}\or{8}{10.1}\or{9}{11.2}%
  \or{10}{12.2}% normalsize
  \or{\@xipt}{13}\or{\@xiipt}{14}\or{\@xivpt}{17}%
  \or{\@xviipt}{20}\or{\@xxpt}{24}}%
\normalsize
\linespacing=\baselineskip

\let\@listI\@listi \@listi

\ifcdr@m@nuscript
  \ifluatex
    \RequirePackageIfExists{fourier-otf}{}
  \else
    \RequirePackageIfExists{fourier}{}
  \fi
  \let\sbseries=\bfseries
  \let\textsb=\textbf
\else
  \ifluatex
    \RequirePackage{amssymb}
    \RequirePackage[Scale=.98]{fourier-otf}
    \let\sbseries=\bfseries
    \let\textsb=\textbf
  \else
    \RequirePackage[expert]{fourier}
    \pdfmapfile{=fourier.map}
    \pdfmapfile{=fourier-utopia-expert.map}
  \fi
\fi

\def\@captionheadfont{\bfseries}
\def\cdr@up{}

\long\def\@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
    \captionseparator\@captionfont\cdr@up\enspace#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%% unnumbered/unnamed captions
\def\silentcaption{%
   \ifx\@captype\@undefined
     \@latex@error{\noexpand\caption outside float}\@ehd
     \expandafter\@gobble
   \else
%     \refstepcounter\@captype
     \expandafter\@firstofone
   \fi
   {\@dblarg{\S@caption\@captype}}%
}
\long\def\S@caption#1[#2]#3{%
  \par
  \addcontentsline{\csname ext@#1\endcsname}{#1}%
    {\protect\numberline{\ }{\ignorespaces #2}}%
  \begingroup
    \@parboxrestore
    \if@minipage
      \@setminipage
    \fi
    \normalsize
    \S@makecaption{\csname fnum@#1\endcsname}{\ignorespaces #3}\par
  \endgroup}
\long\def\S@makecaption#1#2{%
  \setbox\@tempboxa\vbox{\color@setgroup
    \advance\hsize-2\captionindent\noindent
%    \@captionfont\@captionheadfont#1%
    \def\cdr@tmp@{\ignorespaces \ifHy@nesting \hyper@@anchor {\@currentHref }{}\else
      \Hy@raisedlink {\hyper@@anchor {\@currentHref }{\relax }}\fi}%
    \def\cdr@tmp@@{#2}%
%    \@xp\ifx\csname hyper@@anchor\endcsname\relax
    \ifx\cdr@tmp@@\cdr@tmp@\cdr@tmp@\else
    \def\cdr@tmp@{\ignorespaces}%
    \ifx\cdr@tmp@@\cdr@tmp@\else% \@xp\@ifnotempty\@xp{\@cdr#2\@nil}{
%    \captionseparator\@captionfont\cdr@up\enspace
#2
    \fi\fi
    \unskip\kern-2\captionindent\par
    \global\setbox\@ne\lastbox\color@endgroup}%
  \ifhbox\@ne % the normal case
    \setbox\@ne\hbox{\unhbox\@ne\unskip\unskip\unpenalty\unkern}%
  \fi
  % \ifdim\wd\@tempboxa=\z@ % this means caption will fit on one line
  %   \setbox\@ne\hbox to\columnwidth{\hss\kern-2\captionindent\box\@ne\hss}%
  % \else % tempboxa contained more than one line
    \setbox\@ne\vbox{\unvbox\@tempboxa\parskip\z@skip
        \noindent\unhbox\@ne\advance\hsize-2\captionindent\par}%
%  \fi
  \ifnum\@tempcnta<64 % if the float IS a figure...
    \addvspace\abovecaptionskip
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
  \else % if the float IS NOT a figure...
    \hbox to\hsize{\kern\captionindent\box\@ne\hss}%
    \nobreak
    \vskip\belowcaptionskip
  \fi
\relax
}
%
%% Page layout
\pagenumbering{arabic}%
%% 1st page
\def\ps@firstpage{
  \ps@plain
  \def\@oddfoot{{\scriptsize
      ISSN (\if@francais \'electronique\else electronic\fi) : \@Eissn\hfill
      \hypersetup{linkcolor=cdr@accentcolor,urlcolor=cdr@accentcolor}
      \texttt{\url{\journalURL}}
  }}
  \let\@evenfoot\@oddfoot
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
%% Identificiation article 1st page
\def\@logofont{\footnotesize}
\def\cdr@subtitlesep{:}

\def\cdr@head{
  \ifcdr@oldtemplate
    \ifcdr@LTXGrid \vspace*{-2.3cm} \else \vspace*{-1.7cm} \fi
    \bgroup
    \@logofont \noindent
    {\Large\textit{Comptes Rendus\\ \CDRcrasseries}\\[2pt]}%
    \ifcdr@m@nuscript \textbf{Draft} \else
      \ifcdr@Attached
        Supplementary material to the article available at:
      \else \ifcdr@efirst
        \ifx\@dateposted\@empty Not yet published%
        \else Published online: {\selectlanguage{english}\printdate{\@dateposted}}\fi
      \else
        \textbf{\currentyear}, Vol.~\currentvolume\displayissue{, }{, Special Issue }, p.\,\pageinfo
      \fi \fi
      \\\texttt{\printDOI}
    \fi
    \hfill\raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}%
    \ifcdr@Attached\else\\[18bp]%
      \centerline{\rule{.8\textwidth}{1.5bp}}%
    \fi
    \par \egroup
    \ifcdr@Attached \vspace{0.6cm} \fi
  \else
    \vspace*{-3cm}
    \bgroup
      \hspace{-1.5cm}\includegraphics[width=6cm]{CR_logo_h_black.pdf}
      \hfill
      \raisebox{1.2cm}{\begin{minipage}[b][][b]{10cm}
        {\hfill\Large\textit{\currentjournaltitle}\par}
        \hfill
        \ifcdr@m@nuscript
          \textbf{Draft}
        \else
          \ifcdr@Attached
            Supplementary material to the article available at:
          \else
            \ifcdr@efirst
              \ifx\@dateposted\@empty
                \if@francais Pas encore publi\'e \else Not yet published \fi
              \else
                \if@francais En ligne depuis le \else Published online: \fi \printdate{\@dateposted}
              \fi
            \else
              \textbf{\currentyear}, Vol.~\currentvolume\displayissue{, }%
                {, \if@francais{\cdr@loc@numspecial@fr\ }\else{Special issue }\fi}, p.\,\pageinfo
            \fi
          \fi
          \par\hfill\texttt{\printDOI}
        \fi
      \end{minipage}}
      \par \vspace{-2ex}
      \centerline{\color{cdr@accentcolor}\rule{\paperwidth}{1mm}}
    \egroup
  \fi
}

\def\@maketitle@hook{
  \cdr@head
  \ifcdr@epreuves \linenumbers \fi
}
%% Standard pages
\def\ps@headings{%
    \ps@empty
    \def\@evenhead{%
        \rlap{\thepage}{}%\scshape
        \footnotesize\def\lastname####1{{####1}}%
        \hfil
        \def\thanks{\protect\thanks@warning}%
        \TopAuthors{}{}\hfil
    }%
    \def\@oddhead{%
        \let\\\relax
        \hfil
        \def\thanks{\protect\thanks@warning}%
        {\footnotesize\TopAuthors{}{}}\hfil
        \llap{\thepage}{}%
    }%
    \let\@mkboth\cdr@markboth
}
%
\ifnum \currentyear < \z@ \relax \def\currentyear{0000} \fi

\ifcdr@volume \else \pagestyle{headings} \fi
%
\setlength{\@titletopskip}{\topskip}
\setlength{\@titlebotskip}{0\p@}
%% title presentation

\let\overtitlebyhand\relax

\def\CDRtitleSep{~/ }

\cdr@ifeq{\cdr@mode}{bio}{
    \title{Guest editors}
    \alttitle{Rédacteurs invités}
    \let\TopAuthors=\relax
    \NewDocumentCommand {\guesteditor} {mm} {
        \begin{minipage}{.3\hsize}
            \centering
            \includegraphics[width=\hsize]{#2}\\
            \textbf{#1}
        \end{minipage}
    }
}{}

\cdr@var@load {..} {cdr@specialtitle@english} {}
\cdr@var@load {..} {cdr@specialtitle@french} {}
\ExplSyntaxOn
  \def\cdr@setarticletype{
    \prop_get:NnN \cdr_meta_prop {articletype} \l_tmpa_tl
    \if@francais
      \prop_get:NVN \cdr_articletypename_fr_prop \l_tmpa_tl \l_tmpb_tl \l_tmpb_tl
      \ifcdr@showtranslation \,/\, \prop_get:NVN \cdr_articletypename_en_prop \l_tmpa_tl \l_tmpb_tl \emph{\l_tmpb_tl} \fi
    \else
      \prop_get:NVN \cdr_articletypename_en_prop \l_tmpa_tl \l_tmpb_tl \l_tmpb_tl
      \ifcdr@showtranslation \,/\, \prop_get:NVN \cdr_articletypename_fr_prop \l_tmpa_tl \l_tmpb_tl \emph{\l_tmpb_tl} \fi
    \fi
  }
  \def\cdr@setarticletopic{
    \if@francais
      \cdr@topicFR \ifcdr@showtranslation\ifx\cdr@topicEN\@empty\else \,/\, \emph{\cdr@topicEN} \fi\fi
    \else
      \cdr@topicEN \ifcdr@showtranslation\ifx\cdr@topicFR\@empty\else \,/\, \emph{\cdr@topicFR} \fi\fi
    \fi
  }
  \def\@settitle{
    \begin{flushleft}
      \ifcdr@HideArticleType \else \bgroup \Large \cdr@setarticletype \par \egroup \fi
      \bgroup \Large \cdr@setarticletopic \par \egroup

      \ifx\TITREspecial\@empty\else \bgroup % This is part of a thematic issue
        \vspace{3ex} \LARGE
        \ifx\overtitlebyhand\relax
          \if@francais
            \let\cdr@specialtitle@main\cdr@specialtitle@french
            \let\cdr@specialtitle@alt\cdr@specialtitle@english
          \else
            \let\cdr@specialtitle@main\cdr@specialtitle@english
            \let\cdr@specialtitle@alt\cdr@specialtitle@french
          \fi
          \ifx\cdr@specialtitle@main\@empty
            \MissingInfo{Special issue title missing!}
          \else
            \ifcdr@swaptitles\@title\else\cdr@specialtitle@main\fi
            \ifx\cdr@specialtitle@alt\@empty\else
              \ifcdr@showtranslation\CDRtitleSep{\itshape\ifcdr@swaptitles\@alttitle\else\cdr@specialtitle@alt\fi}\fi
            \fi
          \fi
        \else
          \overtitlebyhand
        \fi
      \par \egroup \fi

      \vspace{3ex}

      {\Huge\ifcdr@swaptitles\cdr@specialtitle@english\else
        \@title
        \ifx\@subtitle\@empty\else \if@francais\,\fi :~ \@subtitle\fi
      \fi\par}

      \ifcdr@showtranslation
        { \if@francais\selectlanguage{french}\else\selectlanguage{english}\fi
          \huge\itshape
          \ifx\@alttitle\@empty\else
              \vspace*{14pt}
              \ifcdr@swaptitles\cdr@specialtitle@french\else
                  \ifcdr@Attached
                    \if@francais Supplementary ~ material: \else Document ~ compl\'ementaire\,: \fi ~
                  \fi\@alttitle % TODO French spacing for alt title
                  \ifx\@altsubtitle\@empty\else\if@francais\else\,\fi :~ \@altsubtitle\fi
              \fi
              \par
          \fi}
      \fi

      \vspace*{16pt}
    \end{flushleft}
  }
\ExplSyntaxOff
%

\let\@ESM\@empty
\newcommand\ESM[1]{\def\@ESM{#1}}

\def\cdr@preabstracthook{\par\bigskip}
\def\cdr@interabstracthook{\par}%\smallskip}
\def\cdr@postabstracthook{%
    \@@par\smallskip
    \ifx\@empty\@keywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setkeywords}\smallskip
    \fi
    \ifcdr@showtranslation\ifx\@empty\@altkeywords\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setaltkeywords}\smallskip
    \fi\fi
    \ifx\@empty\@subjclass\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setsubjclass}\smallskip
    \fi
    \ifx\@empty\thankses\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setthanks}\smallskip
    \fi
    \CDRifmeta {note}
    {\@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setnote}\smallskip}
    {}
    \ifx\@empty\@ESM\else
        \@@par\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setESM}\smallskip
    \fi
    \@setpostabstractnotes
    \@@par{\abstractfont\leftskip\abstractmargin\rightskip\leftskip{\parindent\z@\@setdate}\par}
    \bigskip\bigskip
}
%
\def\CDRextrafirstfootnotetext{}
\def\abstractheadfont{\bfseries}
\def\@setabstracthead{{\abstractheadfont\abstractname\unskip.\kern.25em\ignorespaces}}
\def\@setaltabstracthead{{\abstractheadfont\altabstractname\unskip.\kern.25em\ignorespaces}%
}
%
%% authors
\def\@firstauthor#1\and#2\stop{#1}
\def\shortrunauthors{\gdef\@maketitle@shortauthors@hook{\def\topauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
\def\shortrunPDGauthors{\g@addto@macro\@maketitle@shortauthors@hook{\def\PDGauthors{\@xp\@firstauthor\authors\stop\ \etal}}}
 \if@francais
  \def\manuscriptname{Manuscrit}%
  \def\receivedname{re\c cu}%
  \def\revisedname{r\'evis\'e}%
  \def\acceptedname{accept\'e}%
  \def\@@and{et}%
 \else
  \def\manuscriptname{Manuscript}%
  \def\receivedname{received}%
  \def\revisedname{revised}%
  \def\acceptedname{accepted}%
  \def\@@and{and}%
 \fi
%
\AtBeginDocument{\ifx\@daterevised\@dateaccepted\global\cdr@revisedacceptedtrue\fi
\ifx\@datereceived\@dateaccepted\global\cdr@receivedacceptedtrue\fi}
%
%%%%% presentation auteurs
%\def\@@and{\&}
 \def\author@andify{%
   \nxandlist {\unskip ,\penalty-2 \space\cdr@count@hasaddr=\z@\ignorespaces}%
     {\unskip {} \cdr@count@hasaddr=\z@\@@and~}%
     {\unskip {} \penalty-2  \cdr@count@hasaddr=\z@\@@and~}%
 }
% \def\@maketitle@shortauthors@hook{\msia@shortauthor@andify\shortauthors\let\topauthors\shortauthors}
\newcount\cdr@thankcount
\cdr@thankcount\z@
\ifcdr@LTXGrid\else
\def\@alph#1{\ifcase#1\or a\or b\or c\or d\else\@ialph{#1}\fi}
\def\@ialph#1{\ifcase#1\or \or \or \or \or e\or f\or g\or h\or i\or j\or
 k\or l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or
 y\or z\or aa\or bb\or cc\or dd\or ee\or ff\or gg\or hh\or ii\or jj\or
 kk\or ll\or mm\or nn\or oo\or pp\or qq\or rr\or ss\or tt\or uu\or
 vv\or ww\or xx\or yy\or zz\else\@ctrerr\fi}
\fi
\let\IsEqualContrib\relax
\let\IsCorresp\relax
\newcount\ContrA\ContrA=\z@
\newcount\CorrA\CorrA=\z@
\newcount\DeadA\DeadA=\z@
\def\display@orcid#1{%
  \href{https://orcid.org/#1}{%
    \raisebox{.7ex}[0pt][0pt]{\includegraphics[height=1.1ex]{orcid-bw.png}}%
    }~}
\newcount\cdr@count@hasaddr\cdr@count@hasaddr=\z@%
\def\@setauthors{%
  \begingroup
    \hsize=.9\linewidth \raggedright \large \sbseries
    \cdr@listauthors@cras\par
    \cdr@listnoauthors@cras{appendixwriter}{Appendix by }\par
  \endgroup
  \ifnum\CorrA=\z@\else{{
    \def\@thefnmark{{\footnotesize\rule{0pt}{10pt}$*\,$}}%
    \@footnotetext{%
      \def\CDRss{\ifnum\CorrA>\@ne\relax s\fi}%
      \if@francais
        Auteur\CDRss\ correspondant\CDRss
      \else
        Corresponding author\CDRss
      \fi.
      \CDRextrafirstfootnotetext
    }%
  }}\fi
  \ifnum\ContrA=\z@\else{{
    \def\@thefnmark{\rule{0pt}{10pt}$\#\,$}%
    \@footnotetext{%
      \if@francais Contributions \'egales\else Contributed equally\fi.%
    }%
  }}\fi
  \ifnum\DeadA=\z@\else{{
    \def\@thefnmark{\rule{0pt}{10pt}$\dagger\,$}%
    \@footnotetext{%
      \if@francais D\'ec\'ed\'e\else Deceased\fi.%
    }%
  }}\fi
}%
\def\@setafterauthor{%
  \vglue3mm%
%  \hspace*{0pt}%
\begingroup\hsize=10cm\advance\hsize\abstractmarginL\raggedright
\noindent
%\hspace*{\abstractmarginL}\begin{minipage}[t]{10cm}
   \leftskip\abstractmarginL
  \normalfont\Small
  \@afterauthor\par
\endgroup
\vskip2pt plus 3pt minus 1pt
}
\def\@afterauthor{%
    \ifx\@empty\addresses\else
        \@setaddresses\par
        \ifcdr@GroupEmails
            \ifcdr@existcurraddr
                \@setcurraddr\par
            \fi
            \@setemails\par
        \fi
        \bigskip%
    \fi
    \ifx\postaddressinfo\relax\else\textbf{\postaddressinfo}\par\bigskip\fi
}
\newif\ifcdr@existcurraddr\cdr@existcurraddrfalse
\def\@setaddresses{\begingroup
  \cdr@thankcount\z@
  \url@samestyle
  \def\affiliationonly##1{##1}%
  \def\snailmailonly##1{\relax}%
  \def\lastname##1{\relax}%
  \def\firstname##1{\relax}%
  \def\hasthanks##1{##1\@addpunct.\@par}%
  \def\hasaddress##1{\relax}%
  \def\doauthorinfo##1{\@@par\textit{##1}}%
  \def\noauthor##1##2{}%
  \def\author##1{\def\\{ \ignorespaces}\ignorespaces}%
  \def\address##1##2{\begingroup
    \@ifempty{##1}{% cas pas addressSameAs
      \ifnum\cdr@thankcount>\z@\par\vskip4pt\fi\global\advance\cdr@thankcount\@ne
      \textsuperscript{\textit{\@alph\cdr@thankcount}}\kern.2em{\ignorespaces##2\unskip}}{}\endgroup}%
  \def\curraddr##1##2{%% Showing emails authorwise? Let's assume this follows the same logic as emails grouping.
    \ifcdr@GroupEmails\global\cdr@existcurraddrtrue\else\begingroup
      \@ifnotempty{##2}{\@@par\curraddrname{}\textit{\thsp:} %
      {\ignorespaces##2\unskip}\endgroup}\fi}%
  \def\email##1##2{%
    \ifcdr@GroupEmails\else\begingroup
      \@ifnotempty{##2}{\@@par\emailaddrname{}\@ifnotempty{##1}{ (##1)}\textit{\thsp:} \href{mailto:##2}{##2}}%
    \endgroup\fi}%
  \def\urladdr##1##2{\begingroup
    \@ifnotempty{##2}{\@@par\urladdrname{}\textit{\thsp:} %
      \url{##2}}\endgroup}%
  \addresses \endgroup}
\def\@setemails{\begingroup
  \cdr@thankcount\z@
  \url@samestyle
  \def\affiliationonly##1{\relax}%
  \def\snailmailonly##1{\relax}%
  \def\lastname##1{\relax}%
  \def\firstname##1{\relax}%
  \def\hasthanks##1{\relax}
  \def\hasaddress##1{\relax}%
  \def\noauthor##1##2{}%
  \def\author##1{}%
  \def\address##1##2{\relax}%
  \def\curraddr##1##2{\relax}%
  \def\doauthorinfo##1{\relax}%
  \def\email##1##2{%
    \ifcdr@GroupEmails\begingroup
      \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi\href{mailto:##2}{##2}\@ifnotempty{##1}{ \mbox{(##1)}}}%
    \endgroup\fi
    \global\advance\cdr@thankcount\@ne}%
  \def\urladdr##1##2{\relax}%
  \sbox\@tempboxa{\addresses\xdef\CDRess{\ifnum\cdr@thankcount>\@ne\relax s\fi}}%
  \ifdim\wd\@tempboxa>1em\relax
    \vskip2pt\@@par\textit{\emailsaddrname{}\CDRess\thsp:}
    \cdr@thankcount\z@
    \addresses%
  \fi
  \endgroup}
\def\@setcurraddr{%\par
  \begingroup
   \cdr@thankcount\z@
   \url@samestyle
   \def\affiliationonly##1{\relax}%
   \def\snailmailonly##1{\relax}%
   \def\lastname##1{\relax}%
   \def\firstname##1{\relax}%
   \def\hasthanks##1{\relax}
   \def\hasaddress##1{\relax}%
   \def\author##1{}%\ifnum\cdr@thankcount=\z@\else, \fi}
   \def\address##1##2{\relax}%
   \def\doauthorinfo##1{\relax}%
   \def\curraddr##1##2{%% Showing current addresses?
     \ifcdr@GroupEmails
     \begingroup
     \@ifnotempty{##2}{\ifnum\cdr@thankcount=\z@\else, \fi##2\@ifnotempty{##1}{ \mbox{(##1)}}}\endgroup\fi
     \global\advance\cdr@thankcount\@ne}%
   \def\email##1##2{\relax}%
   \def\urladdr##1##2{\relax}%
   \sbox\@tempboxa{\addresses\xdef\CDREss{\ifnum\cdr@thankcount>\@ne\relax es\fi}}%
   \ifdim\wd\@tempboxa>1em\relax
   \vskip2pt\@@par\textit{\curraddrname{}\CDREss\thsp:}
   \cdr@thankcount\z@
   \addresses%\@addpunct.%
   \fi
   \endgroup
 }

\def\@adminfootnotes{}

\def\@setsubjclass{%
  \abstractfont
  {\abstractheadfont\subjclassname.}\kern.25em\ignorespaces
  \@subjclass\@addpunct{{\upshape.}}\par}
\setlist{font=\upshape}
\newif\ifcdr@revisedaccepted\cdr@revisedacceptedfalse
\newif\ifcdr@receivedaccepted\cdr@receivedacceptedfalse
\newif\ifcdr@french@issue@title \cdr@french@issue@titlefalse
\def\daterevisedaccepted#1{%
  \def\@daterevised{#1}%
  \def\@dateaccepted{#1}%
  \cdr@revisedacceptedtrue
}
\def\@setdate{%
  \ifx\@empty\@dateaccepted
    \MissingInfo{This article is a draft (not yet accepted!)}%
  \else
    \if@francais
      \itshape\selectlanguage{french}%
      \noindent Manuscrit re\c cu
      \ifcdr@receivedaccepted
        et accept\'e le \printdate\@datereceived
      \else
        le \printdate\@datereceived,
        \ifcdr@revisedaccepted
          r\'evis\'e et  accept\'e le \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            r\'evis\'e le \printdate\@daterevised
            \ifx\@empty\@datererevised
            \else
              \ et le \printdate\@datererevised
            \fi,
          \fi
          accept\'e le \printdate\@dateaccepted
        \fi
      \fi.
    \else
      \itshape\selectlanguage{english}%
      \noindent Manuscript
      received
      \ifcdr@receivedaccepted
        and accepted \printdate\@datereceived
      \else
        \printdate\@datereceived,
        \ifcdr@revisedaccepted
          revised and  accepted  \printdate\@dateaccepted
        \else
          \ifx\@empty\@daterevised
          \else
            revised \printdate\@daterevised
            \ifx\@empty\@datererevised
            \else
              \ and \printdate\@datererevised
            \fi,
          \fi
          accepted  \printdate\@dateaccepted
        \fi
      \fi.
    \fi
  \fi
}
% Special case for CRBIOL, we display issue date below the abstract
\cdr@ifeq{\cdr@journal}{CRBIOL}{
  \def\@setdate{
    \if@francais
      \itshape\selectlanguage{french}\strut
      \ifx\@dateposted\@empty\else Publication en ligne : \printdate{\@dateposted}\fi
      \ifx\@dateposted\@empty\else\ifx\@datepublished\@empty\else, \fi\fi
      \ifx\@datepublished\@empty\else Publication du numéro : \printdate{\@datepublished}\fi
      \ifx\@dateposted\@empty\ifx\@datepublished\@empty Publication en cours\fi\fi
    \else
      \itshape\selectlanguage{english}\strut
      \ifx\@dateposted\@empty\else Published online: \printdate{\@dateposted}\fi
      \ifx\@dateposted\@empty\else\ifx\@datepublished\@empty\else, \fi\fi
      \ifx\@datepublished\@empty\else Issue date: \printdate{\@datepublished}\fi
      \ifx\@dateposted\@empty\ifx\@datepublished\@empty Not yet published\fi\fi
    \fi
  }
}{}
\ifcdr@Thematic
    % \AtBeginDocument{%
    %     \let\@datereceived\@empty
    %     \let\@daterevised\@empty
    %     \let\@dateaccepted\@empty
    %     \let\@datererevised\@empty
    % }%
    % \def\@setdate{
    %   \if@francais
    %     \itshape\strut
    %     \ifx\@dateposted\@empty\else Publi\'e en ligne le \printdate{\@dateposted}\fi
    %     \ifx\@dateposted\@empty\else\ifx\@datepublished\@empty\else, \fi\fi
    %     \ifx\@datepublished\@empty\else Publication du num\'ero le \printdate{\@datepublished}\fi
    %     \ifx\@dateposted\@empty\ifx\@datepublished\@empty Not yet published\fi\fi
    %   \else
    %     \itshape\strut
    %     \ifx\@dateposted\@empty\else Published online: \printdate{\@dateposted}\fi
    %     \ifx\@dateposted\@empty\else\ifx\@datepublished\@empty\else, \fi\fi
    %     \ifx\@datepublished\@empty\else Issue date: \printdate{\@datepublished}\fi
    %     \ifx\@dateposted\@empty\ifx\@datepublished\@empty Not yet published\fi\fi
    %   \fi
    % }
\fi
%
\def\dedicatoryfont{\normalfont\footnotesize\itshape}
\def\@setdedicatory{%
    \begingroup
      \def\signature##1{\nobreak\hskip 2em plus 1fil
        \penalty-5\hbox{}\nobreak\hfil\parfillskip=0pt
        \mbox{\upshape ##1}\par}
      \raggedleft
      \dedicatoryfont
      \@dedicatory\par
    \endgroup}
\def\@setkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\keywordsname.}\kern.25em\ignorespaces
  \@keywords\unskip\@addpunct{{\upshape.}}\par}
\def\@setaltkeywords{%
  \global\kwd@count=\z@%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\altkeywordsname.}\kern.25em\ignorespaces
  \@altkeywords\unskip\@addpunct{{\upshape.}}\par}
\newcount\cdr@numberofthanks\cdr@numberofthanks=\z@
\def\@setthanks{\abstractfont\def\thanks##1{\ifnum\cdr@numberofthanks=\z@\relax\else\@par
   \fi##1\@addpunct{{\upshape.}}\advance\cdr@numberofthanks1\relax}{\abstractheadfont\thanksname.}\kern.25em\ignorespaces\thankses\par}
\def\@setnote{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\notename.}\kern.25em\ignorespaces
  \CDRgetmeta{note}\@addpunct{{\upshape.}}\par}
\ExplSyntaxOn
  \NewDocumentCommand {\@setpostabstractnotes} {} {
    \bgroup
      \def\do##1##2{{\@@par\noindent\abstractfont {\abstractheadfont##1.}\kern.25em\ignorespaces
        ##2\@addpunct{{\upshape.}}\@@par\smallskip}}
      \seq_map_inline:Nn \cdr_note_seq {##1}
    \egroup
  }
\ExplSyntaxOff
\def\@setESM{%
  \abstractfont%\hskip-\normalparindent
  {\abstractheadfont\ESMname.}\kern.25em\ignorespaces
  \@ESM\@addpunct{{\upshape.}}\par}
\def\@settranslators{\par
  \begingroup
  \translatedby\ \andify\@translators
  {\sl \ignorespaces\@translators} \@@par
  \endgroup}
\if@francais
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Mots-cl{\'e}s}
\def\altkeywordsname{Keywords}
\def\subjclassname{Classification math{\'e}matique par sujets (2010)}
\def\thanksname{Financement}
\def\emailsaddrname{Courriel}
\def\notename{Note}
\def\ESMname{Mat{\'e}riel {\'e}lectronique suppl{\'e}mentaire}
\else
\def\cdr@correspondingname{Correspondance}
\def\keywordsname{Keywords}
\def\altkeywordsname{Mots-cl{\'e}s}
\def\subjclassname{Mathematical subject classification (2010)}
\def\thanksname{Funding}
\def\emailsaddrname{E-mail}
\def\notename{Note}
\def\ESMname{Electronic supplementary material}
\fi
\@xp\let\csname subjclassname@2010\endcsname \subjclassname
%
\def\longthankssection{\subsubsection*{Acknowledgements}}
\long\def\longthanks#1{\longthankssection

  #1}%
%
%
\def\enddoc@text{}
%
%% Page de garde
\def\@makePagedeGarde{
  \ifcdr@epreuves
    \SetWatermarkText{\normalfont PROOFS}
    \setlength\linenumbersep{.2cm}
  \fi
  \ifcdr@pagedegarde
    \ifcdr@traduction
      \input{CR-pagedegarde-traduction}
    \else
      \input{CR-pagedegarde}
    \fi
    \newpage
    \pagecolor{white}\gdef\GPT@pageliteral{}
  \else\ifcdr@epreuves
    \input{CR-pagedemetas}
    \newpage
    \pagecolor{white}\gdef\GPT@pageliteral{}
  \fi\fi
}
%
\ifcdr@sommaire % TODO: perhaps this is useless now
\let\cdr@postabstracthook\@empty
\def\ps@firstpage{\count@=\currentyear
  \ps@plain
  \let\@oddfoot\@empty
  \let\@evenfoot\@oddfoot
  \def\@oddhead{\@serieslogo\hss}%
  \let\@evenhead\@oddhead % in case an article starts on a left-hand page
}
%
\let\ps@headings\ps@empty
\let\ps@plain\ps@empty
\def\article@logo{%
    \set@logo{%
        \hsize\textwidth
        {\Large\textit{Comptes Rendus\\\CDRcrasseries}\\[2pt]}%
        \ifx\@empty\currentvolume
            \textbf{Draft}
        \else
            \textbf{\currentyear},
            \currentvolume
            \ifx\currentissue\@empty\else, \no\currentissue
        \fi\fi\\
        \mbox{}%
        \hfill
        \raisebox{-3mm}[0pt][0pt]{\includegraphics[height=16mm]{Logo_Academie_grisfonce.pdf}}\\[18bp]
        \centerline{\rule{.8\textwidth}{1.5bp}}
    }%
}
%
\def\smfbyname{\vspace*{-17mm}}
\def\lastname#1{#1}
\def\junior#1{\unskip, #1}%
\renewcommand{\@pnumwidth}{4.5em}
\def\@adminfootnotes{}
\def\enddoc@text{}
%%
\fi
\ifcdr@volume
    \cdr@InlineCouvtrue
    \cdr@InlineSomtrue
    \def\cdr@somhook{\small}
    \AtBeginDocument{\hypersetup{linkcolor=cdr@accentcolor,urlcolor=cdr@accentcolor}}
    \def\@makefront{%
        \IncludeSom
        \cleardoublepage
        \ifcdr@SOM
            % The point is to define cdr@resps and so on (for thematic issues)
            % the .cdrsom file is input by CR-couverture.tex
            % TODO this is much too complicated
            \@makeSOM
            \begingroup\makeatletter
                \newcommand\SomLine[9]{%
                    \gdef\cdr@resps{##2}%
                    \gdef\cdr@specialtitle@french{##5}%
                    \gdef\cdr@specialtitle@english{##4}%
                }%
                \InputIfFileExists{\jobname.cdrsom}{%
                    \message{** Fichier  \jobname.cdrsom charge  **^^J}}{%
                    \message{** Pas de fichier \jobname.cdrsom  pour ce volume !**^^J}}%
            \makeatother\endgroup
        \fi
    }
    \def\enddoc@text{}
    \renewcommand{\part}[1]{
        \ifcdr@somfileopen\else
            \immediate\openout\cdr@somfile=\CDRidvol.som
            \cdr@somfileopentrue
        \fi
        \immediate\write\cdr@somfile{\string\somtopic{#1}}

        \cleardoublepage
        \mbox{}
        \vfill
        \begin{center}
          \Huge\bf #1\par
        \end{center}
        \vfill
        \cleardoublepage
        \addtocounter{page}{-2}
    }
    \newcommand{\somtopic}[1]{
        \par\bigskip
        \begin{center}\Large\textsc{#1}\end{center}
        \nobreak
    }
\else % grab special volume editors from parent TODO: use \cdr@var@load for this
  \newcommand\SomLine[9]{
    \gdef\cdr@resps{#2}
    \gdef\cdr@specialtitle@french{#5}
    \gdef\cdr@specialtitle@english{#4}
  }
  \InputIfFileExists{../\CDRidvol.cdrsom}{}{}
\fi

%AJOUTS CS
%\RequirePackage{amssymb,upref}

\NumberTheoremsIn{}
\setcounter{tocdepth}{3}

%% Thms
\ifcdr@ThmDefs\OneNumberAllTheorems\fi
\def\th@plain{%
  \thm@bodyfont{\normalfont\itshape}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em\ignorespaces}%
  \let\thm@indent\noindent
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
  \itshape
}
\def\th@remark{%
  \thm@bodyfont{\normalfont}%
  \thm@headfont{\normalfont\bfseries}%
  \thm@notefont{\normalfont\bfseries}%
  \thm@headpunct{.\kern.2em}%
  \let\thm@indent\noindent
  \def\thm@space@setup{%
    \thm@preskip=\smallskipamount
    \thm@postskip=\thm@preskip}%
}
\let\th@definition\th@plain
%\def\cdr@proofindent{\z@}%{1.5\parindent}
\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\cdr@proofindent
        {\providecommand\printref{\relax}%
\bfseries
    #1\@addpunct{\cdr@proofpunct}}]\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}
%% Sectionning
\def\@startsection#1#2#3#4#5#6{%
 \if@noskipsec \leavevmode \fi
 \par \@tempskipa #4\relax
 \@afterindenttrue
 \ifdim \@tempskipa <\z@ \@tempskipa -\@tempskipa \@afterindentfalse\fi
 \if@nobreak \everypar{}\else
     \addpenalty\@secpenalty\addvspace\@tempskipa\fi
 \@ifstar{\@dblarg{\@sect{#1}{\@m}{#3}{#4}{#5}{#6}}}%
         {\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}%
}
\def\@seccntformat#1{%
  \protect\textup{\protect\@secnumfont
    \csname the#1\endcsname
    \protect\@secnumpunct
  }%
}
\def\@sectionfamily{\normalfont}
\def\@sectionfont{\@sectionfamily\large\bfseries}
\let\contentsnamefont\@sectionfont
\def\@secnumfont{\selectfont}
%\def\@upn{\normalfont\selectfont}
\def\@subsectionfont{\@sectionfamily\large\itshape}
\def\@subsubsectionfont{\@sectionfamily\itshape}
\def\@paragraphfont{\normalfont\bfseries}


\def\section{\@startsection{section}{1}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\@sectionfont}}
\def\subsection{\@startsection{subsection}{2}%
  \z@{-1.5\linespacing\@plus-.5\linespacing\@minus-.5\linespacing}{.8\linespacing\@plus.2\linespacing\@minus.3\linespacing}%
  {\normalfont\@subsectionfont}}
\def\subsubsection{\@startsection{subsubsection}{3}%
  \z@{.5\linespacing\@plus.5\linespacing}{.5\linespacing}%
  {\normalfont\@subsubsectionfont}}
\def\paragraph{\@startsection{paragraph}{4}%
  \z@{.5\linespacing\@plus.5\linespacing}{-\fontdimen2\font}%
  {\normalfont\@paragraphfont}}
%
\newcount\tochyphenpenalty
\tochyphenpenalty\@M
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\tochyphenpenalty
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax
      \advance\leftskip\@tempdima\relax
    \advance\rightskip\@pnumwidth % plus1em
    \parfillskip-\@pnumwidth
    {#5{\leavevmode\hskip-\@tempdima #6}}%
    \nobreak
    \xleaders\hbox to1ex{\normalfont\hss.\hss}\hfil\nobreak
    \hbox to\@pnumwidth{\@tocpagenum{#7}}\par
    \nobreak
    \endgroup
  \fi}
%
\renewcommand{\tocpart}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 #2.\kern1ex}}#3}
\let\tocsection\tocpart
\let\tocsubsection\tocsection
\let\tocsubsubsection\tocsection
\let\tocparagraph\tocsection
\def\l@part{\@tocline{-1}{12pt plus2pt}{0pt}{}{\bfseries\smf@boldmath}}
\def\l@section{\@tocline{1}{0pt}{0pc}{}{}}
\def\l@subsection{\@tocline{2}{0pt}{1pc}{}{}}
\def\l@subsubsection{\@tocline{3}{0pt}{2pc}{}{}}
\def\l@paragraph{\@tocline{5}{0pt}{3pc}{}{}}
\def\l@figure{\@tocline{0}{3pt plus2pt}{0pt}{}{}}
\let\l@table\l@figure
%
\def\@smfprotect{\let\smfcr\\\def\\{\protect\smfcr}}
\DeclareRobustCommand{\MakeUppercase}[1]{{%
    \@smfprotect\upchars@
    \protected@edef\reserved@a{#1}\uppercasenonmath\reserved@a\reserved@a}}
\protected@edef\MakeUppercase#1{\MakeUppercase{#1}}
%
% \def\@makefnmark{%
%   \leavevmode
%   \raise.9ex\hbox{\fontsize\sf@size\z@\normalfont(\@thefnmark)}%
% }%CS
%
%% Additional macros %%
\AtBeginDocument{%
    \csname url@samestyle\endcsname
}
\emergencystretch2em
\arraycolsep 1.5pt
%%
\def\etal{{\normalfont\itshape et al.}}

\def\sautpage{\vadjust{\pagebreak}}
\newcommand\PB{\pagebreak}
\newcommand\SP{\sautpage}
\newcommand\SPB{\sautpage\break}
\newcommand\PBI{\pagebreak\noindent}

\def\orcid@link#1{\href{https://orcid.org/#1}{\includegraphics[height=1.5ex]{orcid-bw.png}}}

\ExplSyntaxOn
\NewDocumentCommand {\displayissue} {mm} {
  \ifx\currentissue\@empty\else
  \exp_args:NV \str_if_in:nnF \currentissue {G}
    {\exp_args:NV \str_if_in:nnTF \currentissue {S} {#2} {#1} \currentissue}
  \fi
}

\NewDocumentCommand {\cdr@typeset@person} {O{author}mm} { % #2 is index, #3 is name
  \bgroup
    \cdr_db_select_index_where_index_eq:Nnnn \l_tmpa_seq {address} {#1} {#2}
    \seq_set_map:NNn \l_tmpb_seq \l_tmpa_seq {\emph{\symbol{\numexpr96+##1}}}
    \seq_clear:N \l_tmpa_seq
    \def\CDRdecoration##1{\unskip\seq_put_right:Nn \l_tmpa_seq {##1}}
    \def\CDRorcid##1{\CDRdecoration{\orcid@link{##1}}}
    \def\IsCorresp{\CDRdecoration{$*$} \global\advance\CorrA\@ne\relax}
    \def\IsEqualContrib{\CDRdecoration{$\#$} \global\advance\ContrA\@ne\relax}
    \def\dead{\CDRdecoration{$\dagger$} \global\advance\DeadA\@ne\relax}
    \def\thanks{\protect\thanks@warning}
    #3
    \seq_map_inline:Nn \l_tmpb_seq {\seq_put_right:Nn \l_tmpa_seq {##1}}
    \seq_if_empty:NF \l_tmpa_seq
      { \, \@textsuperscript{\footnotesize \seq_use:Nn \l_tmpa_seq {,\hspace{.1em}}} }
  \egroup
}

\NewDocumentCommand {\cdr@list@authors} {O{author}} {
  \cdr_db_map_list:nnnnn {#1} { \cdr@typeset@person [#1] {##1} {##2} }
    {~{\@@and}~} {,~} {~{\@@and}~}
}

\def\cdr@listauthors@cras{\cdr@list@authors}

\def\cdr@listnoauthors@cras#1#2{
  \seq_if_in:NnT \cdr_db_contrib_seq {#1} {#2 \cdr@list@authors [noauthor]}
}
\ExplSyntaxOff

\ifluatex
  \babelfont[*cyrillic]{rm}{FreeSerif}
  \babelfont[thai]{rm}{FreeSerif}
\fi

%%%%%%%%% Localization

\def\cdr@loc@redacinv@fr{R\'edacteur\CDRrss\ en chef invit\'e\CDRrss}
\def\cdr@loc@numspecial@fr{Num\'ero sp\'ecial}
